The Hubble Space Telescope Cluster Supernova Survey: V. Improving the Dark Energy Constraints Above z>1 and Building an Early-Type-Hosted Supernova Sample

We present ACS, NICMOS, and Keck AO-assisted photometry of 20 Type Ia supernovae SNe Ia from the HST Cluster Supernova Survey. The SNe Ia were discovered over the redshift interval 0.623 < z < 1.415. Fourteen of these SNe Ia pass our strict selection cuts and are used in combination with the world's sample of SNe Ia to derive the best current constraints on dark energy. Ten of our new SNe Ia are beyond redshift $z=1$, thereby nearly doubling the statistical weight of HST-discovered SNe Ia beyond this redshift. Our detailed analysis corrects for the recently identified correlation between SN Ia luminosity and host galaxy mass and corrects the NICMOS zeropoint at the count rates appropriate for very distant SNe Ia. Adding these supernovae improves the best combined constraint on the dark energy density \rho_{DE}(z) at redshifts 1.0 < z < 1.6 by 18% (including systematic errors). For a LambdaCDM universe, we find \Omega_\Lambda = 0.724 +0.015/-0.016 (68% CL including systematic errors). For a flat wCDM model, we measure a constant dark energy equation-of-state parameter w = -0.985 +0.071/-0.077 (68% CL). Curvature is constrained to ~0.7% in the owCDM model and to ~2% in a model in which dark energy is allowed to vary with parameters w_0 and w_a. Tightening further the constraints on the time evolution of dark energy will require several improvements, including high-quality multi-passband photometry of a sample of several dozen z>1 SNe Ia. We describe how such a sample could be efficiently obtained by targeting cluster fields with WFC3 on HST.

==> figures/figure_b_ltcv_old.tex <==
\ifemapj \begin{figure*}[]
\else \begin{figure}[]
\fi

%\begin{figure}
\begin{center}
\includegraphics[angle=270,scale=.25,width=0.5\columnwidth]{./figures/fig_b_v01_ltcv_01_K000.ps}
\vspace{2mm}
\includegraphics[angle=270,scale=.25,width=0.5\columnwidth]{./figures/fig_b_v01_ltcv_02_G004.ps}
\vspace{2mm}
\includegraphics[angle=270,scale=.25,width=0.5\columnwidth]{./figures/fig_b_v02_ltcv_03_D006.ps}
\vspace{2mm}
\includegraphics[angle=270,scale=.25,width=0.5\columnwidth]{./figures/fig_b_v02_ltcv_04_H005.ps}
\vspace{2mm}
\includegraphics[angle=270,scale=.25,width=0.5\columnwidth]{./figures/fig_b_v01_ltcv_05_R012.ps}
\vspace{2mm}
\includegraphics[angle=270,scale=.25,width=0.5\columnwidth]{./figures/fig_b_v01_ltcv_06_A004.ps}
\vspace{2mm}
\includegraphics[angle=270,scale=.25,width=0.5\columnwidth]{./figures/fig_b_v01_ltcv_07_N033.ps}
\vspace{2mm}
\includegraphics[angle=270,scale=.25,width=0.5\columnwidth]{./figures/fig_b_v01_ltcv_08_F012.ps}
\vspace{2mm}

%\end{center}
%\caption{\NOTE{to be revised : v150}Photometry Data points and light curve fits.} \label{fig:b} \label{fig:ltcv}
%\end{figure}
%\ifemapj \end{figure*}
%\else  \end{figure}
%\fi

%\begin{figure}
%\ifemapj \begin{figure*}[p]
%\else \begin{figure}[p]
%\fi
%\figurenum{\ref{fig:ltcv}}
%\begin{center}
\includegraphics[angle=270,scale=.25,width=0.5\columnwidth]{./figures/fig_b_v01_ltcv_09_C000.ps}
\vspace{2mm}
\includegraphics[angle=270,scale=.25,width=0.5\columnwidth]{./figures/fig_b_v02_ltcv_10_U004.ps}
\vspace{2mm}
\includegraphics[angle=270,scale=.25,width=0.5\columnwidth]{./figures/fig_b_v01_ltcv_11_E012.ps}
\vspace{2mm}
\includegraphics[angle=270,scale=.25,width=0.5\columnwidth]{./figures/fig_b_v01_ltcv_12_D000.ps}
\vspace{2mm}
\includegraphics[angle=270,scale=.25,width=0.5\columnwidth]{./figures/fig_b_v01_ltcv_13_C001.ps}
\vspace{2mm}
\includegraphics[angle=270,scale=.25,width=0.5\columnwidth]{./figures/fig_b_v01_ltcv_14_H003.ps}
\vspace{2mm}
\includegraphics[angle=270,scale=.25,width=0.5\columnwidth]{./figures/fig_b_v01_ltcv_15_P009.ps}
\vspace{2mm}
\includegraphics[angle=270,scale=.25,width=0.5\columnwidth]{./figures/fig_b_v01_ltcv_16_Z005.ps}
\vspace{2mm}
\end{center}
%\caption[]{\NOTE{fig:b}}
\caption{\NOTE{fig:b to be revised : v150} 20 \sneia light curve fits by SALT2.
Flux is normalized to the \zacs-band zeropoint magnitude. 
ACS \iacs, ACS \zacs and NICMOS F110W data is color coded in blue, green and
red respectively.  Note, SCP~05D06 (z=1.314) has $H$-band data from Keck AO system (orange)
\citep{melbourne07a} and they are consistent with HST/ACS and HST/NICMOS light curve fit data.
} \label{fig:b} \label{fig:ltcv}
%\end{figure}

\ifemapj \end{figure*}
\else  \end{figure}
\fi



==> figures/figure_i01_hubblebinindiv.tex <==
\thispagestyle{empty}
\begin{sidewaysfigure}
%% An update of Figure~8 from~K08 where the data from this work
%% has been added, together with other data sets that has recently
%% been published.
%%
\centering
\includegraphics[width=0.75\textheight,angle=90]{%
  ./figures/fig_i01v04_hubblebinindiv.eps}
\caption{\NOTE{fig:i01}Individual diagrams and distributions for the different data
  sets. From left to right: a) Hubble diagram for 
  each sample; b) binned magnitude residuals from the best-fit
  cosmology (bin-width: $\Delta z = 0.01$); c) unbinned magnitude
  residuals from the best fit; d) histogram of the residuals from the
  best fit; e) pull of individual SNe as a function of redshift; f)
  histogram of pulls; g) \sn color as a function of redshift; h)
  uncertainty of the color measurement as an illustration of the
  photometric quality of the data. %
  \label{fig:i01}}
\end{sidewaysfigure}



==> figures/figure_i06_omegam_vs_w_snonly.tex <==
\ifemapj \begin{figure*}[]
\else \begin{figure}[]
\fi
%\begin{figure}
\includegraphics[width=0.45\textwidth]{%
  ./figures/fig_i06av04_omegam_vs_w_snonly_stat.eps}%
\hspace{0.06\textwidth}%
\includegraphics[width=0.45\textwidth]{%
  ./figures/fig_i06bv04_omegam_vs_w_snonly_sys.eps}%
\caption{\NOTE{fig:i06}$68.3\%$, $95.4\%$, and $99.7\%$ confidence regions of the
  $(\omegam,w)$ plane from \sne alone from K08 (dashed contours) and this
  compilation (shaded contours). Systematic errors are included in the
  right panel. Zero curvature has been assumed.
  \label{fig:i06}}
%\end{figure}
\ifemapj \end{figure*}
\else  \end{figure}
\fi



==> figures/figure_l01_acsdxdy.tex <==
\begin{figure}[p]
\begin{center}
\includegraphics[angle=0,scale=.75,width=0.75\textwidth]{./figures/fig_l01v01_acsdxdy.ps}
\end{center}
\caption{\NOTE{to be revised : place holder} The size of pixel offset} \label{fig:l01} 
\end{figure}


==> tables/table_g_binsfit2.tex <==
\ifemapj \begin{deluxetable*}{ll|rrrl}
\else \begin{deluxetable}{ll|rrrl}
\fi

  \tablecaption{ Constraints on binned density and equation of state. The
  constraints are computed including BAO, $H_0$, and CMB data. {\bf NS proposes to rewrite the Table \ref{tbl:binnedcosmo} in this way} THIS TABLE IS OBSOLETE!}
      \tablehead{
      \colhead{} & 
      \colhead{} & 
      \colhead{z $<$ 0.5} &
      \colhead{0.5 $<$ z $<$ 1.0} &
      \colhead{1.0 $<$ z $<$ 1.6} &
      \colhead{z   $>$ 1.6 \tablenotemark{a} } }
  %\startdata
  $w$(z)               & (stat only)  & $-1.052^{+0.062}_{-0.065}$ & $-0.77^{+0.58}_{-0.70}$   & $-3.0^{+5.8}_{-3.0}$   &  $<$ 0.0 \\
                         & (w/ sys.)    & $-1.049^{+0.114}_{-0.116}$ & $-0.63^{+0.79}_{-1.02}$   & $-3.3^{+6.8}_{-4.1}$   &  $<$ 0.0 \\
  \hline
  $\rho_{\Lambda}(z) / \rho _{0}$ & (stat only)  & $0.732^{+0.014}_{-0.015}$  & $0.750^{+0.176}_{-0.164}$ & $0.64^{+1.63}_{-0.95}$ &  $<$ 2.0 \\
                         & (w/ sys)     & $0.727^{+0.015}_{-0.016}$  & $0.80^{+0.23}_{-0.21}$    & $0.72^{+0.51}_{-0.44}$ &  $<$ 2.5 
  \enddata
\tablecomments{Constraints on binned $\rho_{\Lambda}(z)/\rho_{0}$ and $w(z)$. 
This redshift binning corresponds to the middle panel of Figure \ref{fig:binnedw} and the right panel of Figure \ref{fig:binnedrho}}
\tablenotetext{a}{We note that there is no observational constraints beyond z$>$1.6}
\ifemapj \end{deluxetable*}
\else  \end{deluxetable}
\fi


==> tables/table_g_binsfit_backup.tex <==
\ifemapj \begin{deluxetable*}{ll}
\else \begin{deluxetable}{ll}
\fi
  \tablecaption{ Constraints on binned density and equation of state. The
  constraints are computed including BAO, $H_0$, and CMB data.
    \label{tbl:binnedcosmo}}
      \tablehead{
    \colhead{SNe} & \colhead{Constraint} }
  \startdata
\hline
Stat Only: & $ \rho_{z < 0.5} =  0.732^{+0.014}_{-0.015} $ $ \rho_{0.5 < z < 1.0} =  0.748^{+0.174}_{-0.163} $ $ \rho_{1.0 < z} =  0.72^{+0.48}_{-0.41} $\\ 
w/ Sys: & $ \rho_{z < 0.5} =  0.727^{+0.015}_{-0.016} $ $ \rho_{0.5 < z < 1.0} =  0.80^{+0.23}_{-0.21} $ $ \rho_{1.0 < z} =  0.72^{+0.51}_{-0.44} $\\ 
\hline
Stat Only: & $ \rho_{z < 0.5} =  0.732^{+0.014}_{-0.015} $ $ \rho_{0.5 < z < 1.0} =  0.750^{+0.176}_{-0.164} $ $ \rho_{1.0 < z < 1.6} =  0.64^{+1.63}_{-0.95} $ $ \rho_{1.6 < z} =  0.84^{+1.98}_{-1.52} $\\ 
w/ Sys: & $ \rho_{z < 0.5} =  0.727^{+0.015}_{-0.016} $ $ \rho_{0.5 < z < 1.0} =  0.80^{+0.23}_{-0.21} $ $ \rho_{1.0 < z < 1.6} =  1.3^{+3.3}_{-1.5} $ $ \rho_{1.6 < z} =  0.0^{+2.4}_{-1.7} $\\ 
\hline
\hline
Stat Only: & $ w_{z < 0.5} =  -1.049^{+0.062}_{-0.064} $ $ w_{0.5 < z < 1.0} =  -0.81^{+0.57}_{-0.66} $ $ w_{1.0 < z} =  -1.07^{+0.70}_{-2.66} $\\ 
w/ Sys: & $ w_{z < 0.5} =  -1.054^{+0.113}_{-0.115} $ $ w_{0.5 < z < 1.0} =  -0.61^{+0.78}_{-0.95} $ $ w_{1.0 < z} =  -1.3^{+1.0}_{-4.1} $\\ 
\hline
Stat Only: & $ w_{z < 0.5} =  -1.052^{+0.062}_{-0.065} $ $ w_{0.5 < z < 1.0} =  -0.77^{+0.58}_{-0.70} $ $ w_{1.0 < z < 1.6} =  -3.0^{+5.8}_{-3.0} $ $ w_{1.6 < z } < 0.11 $\\ 
w/ Sys: & $ w_{z < 0.5} =  -1.049^{+0.114}_{-0.116} $ $ w_{0.5 < z < 1.0} =  -0.63^{+0.79}_{-1.02} $ $ w_{1.0 < z < 1.6} =  -3.3^{+6.8}_{-4.1} $ $ w_{1.6 < z } < 0.14 $\\ 
\hline
Stat Only: & $ w_{z < 0.07} =  -0.70^{+0.36}_{-0.37} $ $ w_{0.07 < z < 0.2} =  -1.37^{+0.33}_{-0.33} $ $ w_{0.2 < z < 0.5} =  -0.83^{+0.32}_{-0.34} $ $ w_{0.5 < z < 1.0} =  -1.01^{+0.74}_{-0.85} $ $ w_{1.0 < z} =  -1.08^{+0.75}_{-3.20} $\\ 
w/ Sys: & $ w_{z < 0.07} =  -0.79^{+0.49}_{-0.49} $ $ w_{0.07 < z < 0.2} =  -1.36^{+0.36}_{-0.36} $ $ w_{0.2 < z < 0.5} =  -0.73^{+0.39}_{-0.41} $ $ w_{0.5 < z < 1.0} =  -1.06^{+0.99}_{-1.23} $ $ w_{1.0 < z} =  -1.1^{+0.9}_{-3.9} $ \\
\hline
\hline
Stat Only (no cluster): & $ \rho_{z < 0.5} =  0.729^{+0.014}_{-0.015} $ $ \rho_{0.5 < z < 1.0} =  0.723^{+0.183}_{-0.169} $ $ \rho_{1.0 < z < 1.6} =  0.69^{+2.34}_{-1.17} $ $ \rho_{1.6 < z} =  0.8^{+2.4}_{-1.8} $\\ 
Stat Only: & $ \rho_{z < 0.5} =  0.728^{+0.014}_{-0.015} $ $ \rho_{0.5 < z < 1.0} =  0.688^{+0.172}_{-0.160} $ $ \rho_{1.0 < z < 1.6} =  1.27^{+2.20}_{-1.22} $ $ \rho_{1.6 < z} =  0.33^{+1.89}_{-1.44} $\\ 
\hline
Stat Only (no cluster): & $ w_{z < 0.5} =  -1.030^{+0.062}_{-0.065} $ $ w_{0.5 < z < 1.0} =  -0.96^{+0.66}_{-0.84} $ $ w_{1.0 < z < 1.6} =  -2.7^{+6.3}_{-2.8} $ $ w_{1.6 < z } < 0.09 $\\ 
Stat Only: & $ w_{z < 0.5} =  -1.025^{+0.062}_{-0.066} $ $ w_{0.5 < z < 1.0} =  -1.11^{+0.75}_{-0.79} $ $ w_{1.0 < z < 1.6} =  1.6^{+2.6}_{-6.6} $ $ w_{1.6 < z } < 0.08 $
\enddata
\ifemapj \end{deluxetable*}
\else  \end{deluxetable}
\fi
